Estimates of the social cost of carbon have increased over time

A meta-analysis of published estimates shows that the social cost of carbon has increased as knowledge about climate change accumulates. Correcting for inflation and emission year and controlling for the discount rate, kernel density decomposition reveals a non-stationary distribution. In the last 10 years, estimates of the social cost of carbon have increased from $33/tC to $146/tC for a high discount rate and from $446/tC to $1925/tC for a low discount rate. Actual carbon prices are almost everywhere below its estimated value and should therefore go up.

==> chi.tex <==
\begin{tabular}{|l|c|c|}
\hline
&\textbf{$\chi_{20}^2$}&\textbf{p}\\\hline
\textbf{All}&12.7726&0.8869\\\hline
\textbf{PRTP = 0\%}&0.9577&1.0000\\\hline
\textbf{PRTP = 1\%}&7.8782&0.9926\\\hline
\textbf{PRTP = 2\%}&16.3455&0.6950\\\hline
\textbf{PRTP = 3\%}&13.8335&0.8388\\\hline
\end{tabular}
